Federated PCA on Grassmann Manifold for IoT Anomaly Detection

With the proliferation of the Internet of Things (IoT) and the rising interconnectedness of devices, network security faces significant challenges, especially from anomalous activities. While traditional machine learning-based intrusion detection systems (ML-IDS) effectively employ supervised learning methods, they possess limitations such as the requirement for labeled data and challenges with high dimensionality. Recent unsupervised ML-IDS approaches such as AutoEncoders and Generative Adversarial Networks (GAN) offer alternative solutions but pose challenges in deployment onto resource-constrained IoT devices and in interpretability. To address these concerns, this paper proposes a novel federated unsupervised anomaly detection framework, FedPCA, that leverages Principal Component Analysis (PCA) and the Alternating Directions Method Multipliers (ADMM) to learn common representations of distributed non-i.i.d. datasets. Building on the FedPCA framework, we propose two algorithms, FEDPE in Euclidean space and FEDPG on Grassmann manifolds. Our approach enables real-time threat detection and mitigation at the device level, enhancing network resilience while ensuring privacy. Moreover, the proposed algorithms are accompanied by theoretical convergence rates even under a subsampling scheme, a novel result. Experimental results on the UNSW-NB15 and TON-IoT datasets show that our proposed methods offer performance in anomaly detection comparable to nonlinear baselines, while providing significant improvements in communication and memory efficiency, underscoring their potential for securing IoT networks.

==> other_packages.tex <==
%\usepackage[pdftex]{graphicx} % Required for including pictures
%\usepackage[pdftex,linkcolor=black,pdfborder={0 0 0}]{hyperref} % Format links for pdf
\usepackage{calc} % To reset the counter in the document after title page    
\usepackage{enumitem} % Includes lists

\usepackage{parskip}

% \usepackage[all]{nowidow} % Tries to remove widows
%\usepackage[protrusion=true,expansion=true]{microtype} % Improves typography, load after fontpackage is selected
\usepackage{algorithm}% http://ctan.org/pkg/algorithm
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx


\usepackage{times}
\usepackage{soul}
\usepackage{url}

\usepackage{setspace}
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
%\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage[detect-all]{siunitx}

\usepackage{xspace}
%\usepackage{caption}
\usepackage{subcaption}
\usepackage{bm}
\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%Multi-line for Algorithm
\usepackage{algorithm,tabularx}
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}
\makeatletter
\newcommand{\multilines}[1]{%
	\begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
		#1
	\end{tabularx}
}
\makeatother

\usepackage{mathtools}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclareMathOperator{\myspan}{span}

\usepackage{amsthm}
\usepackage{multirow}
\usepackage{color}
\usepackage{epstopdf}
\usepackage{endnotes}
\usepackage{framed}
%\usepackage[keeplastbox]{flushend}
\usepackage{cool} % for partial derivative
\usepackage{enumerate} % for \begin{enumerate}[(a)], or [a)]
	%\usepackage{hyperref}
	%\usepackage{url}
	\usepackage[subnum]{cases}
	\usepackage{multicol}
	\usepackage{tablefootnote}
	
	% Special Defined Notation
	\DeclareMathOperator*{\argmax}{arg\,max}
	\DeclareMathOperator*{\argmin}{arg\,min}
	
	\newcommand{\note}[1]{\emph{\color{blue}#1}}
	\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.99mu#1\mkern-1.5mu}\mkern 1.5mu}
	
	\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}
	\DeclarePairedDelimiterX{\abs}[1]{\lvert}{\rvert}{#1}
	\DeclarePairedDelimiterX{\innProd}[1]{\langle}{\rangle}{#1}
	\DeclarePairedDelimiter\set{\lbrace}{\rbrace}
	
	\newcommand{\Prob}[1]{\ensuremath{\mathbb{P} \left[ #1 \right]}}
	\newcommand{\Ex}[1]{\ensuremath{\mathbb{E} \left[ #1 \right]}}
	\newcommand{\Avg}[2]{\ensuremath{\mathbb{E}_{#1} \left[ #2 \right]}}
	\newcommand{\La}[1]{\ensuremath{#1^{*}(s)}} %Laplace transform
	\newcommand{\PrimeN}[2][f]{\ensuremath{#1^{\prime #2}} \,}
	\newcommand{\SumNoLim}[2]{\ensuremath{\sum\nolimits_{#1}^{#2}}}
	\newcommand{\SumLim}[2]{\ensuremath{\sum\limits_{#1}^{#2}}}
	\newcommand{\Setm}[2]{\ensuremath{\{\,#1\mid#2\,\}} \,}
	\newcommand{\defeq}{\vcentcolon=}
	% similarly: \coloneqq
	\newcommand{\eqdef}{=\vcentcolon}
	% similarly: \eqqcolon
	\newcommand*\mean[1]{\bar{#1}}
	\newcommand{\mul}{\ensuremath{\,} \,}
	\newcommand{\pder}[2][]{\frac{\partial#1}{\partial#2}} % use: \pder[f]{x} and \pder{x} where f is optional
	
	\newcommand{\LeRiP}[1]{\ensuremath{\left(#1\right)}}
	\newcommand{\LeRiS}[1]{\ensuremath{\left[#1\right]}}
	\newcommand{\LeRiC}[1]{\ensuremath{\left\{#1\right\}}}
	\newcommand{\nbigP}[1]{\ensuremath{(#1)}}
	\newcommand{\nbigS}[1]{\ensuremath{[#1]}}
	\newcommand{\nbigC}[1]{\ensuremath{\{#1\}}}
	\newcommand{\bigP}[1]{\ensuremath{\bigl(#1\bigr)}}
	\newcommand{\bigS}[1]{\ensuremath{\bigl[#1\bigr]}}
	\newcommand{\bigC}[1]{\ensuremath{\bigl\{#1\bigr\}}}
	\newcommand{\biggP}[1]{\ensuremath{\biggl(#1\biggr)}}
	\newcommand{\biggS}[1]{\ensuremath{\biggl[#1\biggr]}}
	\newcommand{\biggC}[1]{\ensuremath{\biggl\{#1\biggr\}}}
	\newcommand{\BigP}[1]{\ensuremath{\Bigl(#1\Bigr)}}
	\newcommand{\BigS}[1]{\ensuremath{\Bigl[#1\Bigr]}}
	\newcommand{\BigC}[1]{\ensuremath{\Bigl\{#1\Bigr\}}}
	\newcommand{\BiggP}[1]{\ensuremath{\Biggl(#1\Biggr)}}
	\newcommand{\BiggS}[1]{\ensuremath{\Biggl[#1\Biggr]}}
	\newcommand{\BiggC}[1]{\ensuremath{\Biggl\{#1\Biggr\}}}
	% \bigm|, \Bigm|, \biggm|, and \Biggm|
	%%%%% Font commands
	\newcommand{\tbf}[1]{\textbf{#1}}% text bold
	\newcommand{\tit}{\textit}% text italic
	\newcommand{\tsl}{\textsl}% text slanted
	\newcommand{\tsc}{\textsc}% text small cap
	\newcommand{\ttt}{\texttt}% text typewriter
	\newcommand{\trm}{\textrm}% text roman
	\newcommand{\tsf}[1]{\textsf{#1}}% text sans serif
	\newcommand{\tup}{\textup}% text upright
	\newcommand{\mbf}{\mathbf}% math bold
	\providecommand{\mit}{\mathit}% math italic
	\newcommand{\msf}{\mathsf}% math sans serif
	\newcommand{\mrm}{\mathrm}% math roman
	\newcommand{\mtt}{\mathtt}% math typewriter
	\newcommand{\mybold}[1]{\ensuremath{\boldsymbol{#1}}}
	
	\newcommand{\centered}[1]{\begin{tabular}{l} #1 \end{tabular}} 
	
	\newcommand{\Bold}[1]{\boldsymbol{#1}} % Bold math symbol, use as \Bold{\alpha}
	\newcommand{\Cal}[1]{\mathcal{#1}} % phics - only caps, use as \Cal{A}
	\newcommand{\DD}[1]{\mathbb{#1}} % Doubled - blackboard bold - only caps, use as \DD{A}
	%\newcommand{\Euler}[1]{\mathscr{#1}} % Euler Script - only caps, use as \Euler{A}
	\newcommand{\Frak}[1]{\mathfrak{#1}} % Fraktur, use as \Frak{a}
	\newcommand{\blue}[1]{{\color{blue}#1}\xspace}
	\newcommand{\red}[1]{{\color{red}#1}\xspace}
	
	\theoremstyle{plain}
	\newtheorem{theorem}{Theorem}
	\newtheorem{assumption}{Assumption}
	\newtheorem{corollary}{Corollary}
	\newtheorem{lemma}{Lemma}
	\newtheorem{proposition}{Proposition}
	\theoremstyle{definition}
	\newtheorem{definition}{Definition}
	\newtheorem{remark}{Remark}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
